Testing General Relativity with NuSTAR data of Galactic Black Holes : II

General relativity predicts the spacetime metric around an astrophysical black hole to be described by the Kerr solution, which is a massive rotating black hole without any residual charge. In a previous paper, we analyzed the NuSTAR observations of six X-ray binaries to obtain constraints on the deformation parameter $\alpha_{13}$ using a state-of-the-art relativistic model. In this work, we continue analyzing NuSTAR observations of four more X-ray Binaries; two of which, namely Swift~J174540.7--290015 and Swift~J174540.2--290037 are X-ray Transients very close to the supermassive black hole at the center of our galaxy. The other two sources have complicated absorption, which is accounted for by time- and flux-resolved spectroscopy. The observation of MAXI J1631-479 is divided into two parts to account for the sudden increase in flux. The V404 Cygni spectra, obtained by combining two consecutive observations, are divided into 5 flux states and also account for absorption by quantifying the excess flux in the energy range of 6.5-7.0 keV. The constraints obtained are consistent with the Kerr hypothesis and are comparable with those obtained in previous studies and those from gravitational events. This work shows that even highly absorbed sources can be used for testing the Kerr hypothesis, which is possible with careful data reduction and subsequent data analysis.

==> response_to_referee.tex <==
Dear Editor, 

Thank you very much for providing a report for our manuscript. Based on the referee’s suggestions, we have made appropriate modifications in the manuscript which is in red to facilitate the review process. The response of the referee’s comment is also attached with the revised manuscript. WE also attached two figures for one of the referee's comments (Point 10). We sincerely hope that the revised manuscript now meets the standard of publication in the Publications of the Astronomical Society of Japan. 

Yours sincerely, 
Authors


Referee report on “Testing General Relativity with NuSTAR data of Galactic Black Holes: II” 
The paper expands on the analysis of previous work to analyze NuSTAR observations of four galactic black hole systems (during outbursts) to constrain deviations from the Kerr metric, using the relxill_nk models. 
The paper has already received one round of suggestions from a different reviewer. In the updated draft, the authors have partially addressed the comments in that report. 
In particular: 
	1. Regarding the degeneracy between alpha_13 and the spin: the paper reports extremely small uncertainties on the measured BH spin and alpha_13. The paper states that the uncertainties are only statistical and do not include systematic uncertainties. It is not clear that even just the magnitude of the statistical uncertainties is completely demonstrated, seeing how degeneracies between other parameters are not properly quantified. For example, in the analysis of many of the sources, the inner emissivity profile was fixed at 10, the outer emissivity fixed at 3, and the breaking radius allowed to vary. The paper finds that the breaking radius often takes small values. By design, the models aim to make the breaking radius greater than the size of the ISCO. By making q_1=10, the models attempt to reduce its influence to match the observed reflected flux, and decrease r_br, which in turn serves to reduce the size of the ISCO and increases the spin. For example, in lines 525-526, the authors mention that the measured breaking radius is as low as 1.5 r_g. For a spin of 1, the ISCO radius would be 1 r_g (and larger for a spin of 0.996), giving the inner emissivity index a very small area to have an influence over. Furthermore, the inclination and spin act simultaneously on the shape of the Fe line (admittedly, on the opposite sides of the line), and the inclination is known to be correlated with the ionization, Fe abundance, reflection fraction, disk density, etc. (see, e.g., Draghis et al. 2025). 
    
	Response: In this work, statistical error refers to the error obtained by MCMC analysis.  Some of these degeneracies shown in MCMC results are intrinsic to the relxill model. For instance, the model assumes that the inner edge of the disk is at ISCO. So, it will affect other parameters to support this assumption. The reason why some parameters are fixed in the analysis is because their variation is insensitive to the fits and is unconstrained. So, we fix it at a reasonable value, and the effect of such parameters on the fit is also checked with MCMC simulations, where the parameter is found to vary across the whole range. q_1=10 is a reasonable value found in the X-ray analysis of other X-ray binaries in the literature. Also, if we keep q_1 free, it will be pegged to 10, and rbr cannot be constrained. As the aim of this paper is to measure deformation parameter, we discussed its correlations with spin and inclination at appropriate subsections. 
    
	2. Lack of evidence for a warm absorber: The updated manuscript includes a paragraph in the discussion (lines 614-625) that talks about the improvement in chi2 when adding the XSTAR grid to the models. I consider that this explanation should be part of the appropriate subsections (3.3 and 3.4). Still, the figures do not demonstrate the need for this addition to the model. Currently, Figure 3 plots “eeufspec”, which convolves the data with the model, making all apparent features more “impressive”. I recommend demonstrating the need for the warm absorber by plotting the data using “ldata” or “eedata” in xspec, and also showing the residuals produced by the model when the warm absorber is not included in the model. This is along the lines of what Figure 11 attempts to do, but does not accomplish convincingly.  
    
    Response: The warm absorber is added because it improves the chi-square and provides physical and constrained values of some parameters such as ionization parameter. It is also employed when the same observation is analyzed with the Kerr metric in recent literature. The effect of warm absorber on the fit is too small to see it in any residual or eedata plot. We plot eeufspec because it makes the features, as referee mentioned, "impressive". For these reasons, we request the referee to let us keep these eeufspec plots in the paper. 
    
	3.	Assumption of disk extending to the ISCO in the hard state: the updated manuscript adds a sentence talking about that, simply stating it as an assumption. At the very least, some references are needed to back up this assumption. However, in the analysis of MAXI J1631 (lines 322-324), the paper states that the observations in the hard state were not analyzed because they captured the source in the hard state, where the disk is supposedly truncated. This is an inconsistency that needs to be addressed. 
    
    Response : References are added on line 710. The observation is not analyzed because the disk is in a truncated state, which violates the important assumption about ISCO. We fix this inconsistency in the text (lines 349-352). 
    
     The other comments from the initial referee were reasonably addressed. 
     However, before considering this updated manuscript for publication, I consider that a number of additional issues need to be addressed. In the list below, I articulate a few major points, followed by a number of minor points. 
	1.	The paper does not justify its contribution to the field. Prior to this paper, a number of measurements of alpha_13 existed from other papers. This paper provides 4 more, which, according to the results, appear not to change any already existing conclusions. How does this paper enhance the field? Why is it important? How does adding 4 more measurements strengthen any claims? How many more measurements do we really need for any important conclusions? 
    
    Response: This paper attempts to test the Kerr metric for sources with heavy absorption. Until now, only simple sources have been selected for such studies. In this paper, we analyze the absorbed sources and demonstrate that the Kerr metric can be tested if the data of highly absorbed sources are reduced and analyzed carefully. These four measurements would open the new frontier, where the absorbed sources can also be used for such studies. We have found that the deformation shown by the observations observed so far is consistent with the Kerr hypothesis. If not the non-Kerr, it strengthens the claim of these objects being described by the Kerr metric, which is also a confirmation of the assumption of explaining the space-time metric with Kerr in most of the relativistic reflection models in X-ray astronomy. We have included some text in the last section (lines 747-759). 
    
	2.	The paper does not provide adequate justification for how the sources were selected. It is said that the sources were taken from a table in a paper from 2021. That table is not exhaustive, and recent papers have provided much more comprehensive lists of sources analyzed (again, see Draghis et al. 2024, 2025). Furthermore, the paper does not justify why these four complicated sources were chosen for this analysis and, because of their complexity, one could argue that the measurements are even less trustworthy. In lines 533-535, the paper states that such constraints can only be obtained through advanced reduction techniques. First, this claim needs to be expanded upon and argued for. Second, why bother with such complicated spectra when there are more than 200 observations of other sources, many of which show stronger reflection features, better spectral signal to noise, less complexity (flares, absorption), etc. 
    
	Response: The sources are highly absorbed sources and have the spin measurement with the observations we analyzed in this paper. If we have a spin measurement with these highly absorbed sources, then it is also possible to test the Kerr hypothesis.  In Marinucci et al. 2015, the highly variable nature of the source is quantified by dividing the spectra into time intervals for which the variability is constant. In this paper, a similar kind of reduction is done to properly assess the variability before constraining spin. With these 4 sources, we demonstrate that highly variable data can also be used for such study if the data is reduced appropriately. We have added this explanation in Sec. 2 (lines 124-137).  
    
	4.	The paper does not provide adequate justification for the requirement of deviations from the Kerr metric from a spectral perspective. In particular, the paper does not demonstrate that the spectra show any evidence of deviations from the Kerr metric. A naive chain of thought could work as follows: if spectra are well fit with a model that uses the Kerr metric, when using a different model that simplifies to the Kerr metric when one parameter is turned to zero, if all the other parameters are consistent with the measured values using the Kerr metric, it is intuitive that the solutions are the same and that the model will work to bring deviations to zero. A few experiments that would help justify this effort would be to fit the spectra with the same models, but fix the alpha parameter to zero, and check the statistical improvement that comes by allowing alpha to vary. Is it justified (from a statistical perspective) to allow alpha to vary? Can the data really constrain it? If the chi2 is the same with alpha frozen at zero and with alpha varying, then this is not a measurement, but rather proof that the models converge to the same solution. Another possibility is to fix the alpha value at some values (-1, 1, etc) and attempt to find similar solutions (in terms of chi2). What is required for that to work? Do the models need absurd spins and nonphysical Fe abundances, reflection fractions, and emissivity profiles? The paper needs to justify the robustness of its measurements. 
    
    Response: For each source, we first fit the data with alpha_13=0. Each time, the chi-square improves, although less. We have compared the chi-square of relxill\_nk with alpha_13 = 0 and included it in the appropriate subsections. As the value of the deformation parameter always includes the Kerr solution, the solution of Kerr and non-Kerr model will not differ much in terms of chi-square. We have added this in the text (643-651). 
    
    4. The paper does not fully explore the possible impact of parameter correlations on the measurements. This makes the sizes of the uncertainties on the BH spin and on the alpha parameter strongly underestimated. For example, based on Figure 9, the deviations from the Kerr metric would produce effects similar to those of adjusting the reflection fraction in the spectra. This degeneracy needs to be explored. While the paper provides a number of corner plots, these currently serve the purpose of assessing the uncertainties on the parameters rather than exploring the shape of the parameter space. Given the complexity of the data, it is likely that the solution (combination of parameters) is simply stuck in a minimum, and the MCMC would not want to “leave” that region of the parameter space in its exploration, leading to artificially small uncertainties. This is the case especially when the model becomes extremely complicated (such as when including relxill or xstar). This is not to say that the paper needs to include complete corner plots, but rather to improve the exploration of the parameter space. As an example, what happens if the same combination of parameters is taken and directly applied to the relxillCp model (not _nk)? How do the corner plots look like? 
    
    Response: The data were fitted with the different models using the chi-square likelihood in XSPEC. After getting the best fit, the MCMC simulations are done with 500 walkers and 12,000 iterations, which is equivalent to 6 million simulations. The number of walkers is chosen so that the whole physical range of all parameters is explored simultaneously. In the case of part II of MAXI J1631, spin is negatively correlated with the deformation parameter, but has a negative correlation with inclination, which is also similar to the results of part I. Interestingly, for V404, the spin is found to have negligible correlation with other parameters. For T15 and T37, the spin is positively correlated with the inclination but has negative correlation with $\alpha_{13}$ for negative values. For positive values, the correlation is positive for both sources, which also holds for the part I observation of MAXI J1631. These correlations would underestimate the error provided by MCMC simulations, which should be understood with caution. We have added this explanation in the discussion section (lines 665-678). 

    
    Minor Points
    1. Lines 128-129: the paper mentions using nustardas 2.0.0 and name it as the “latest version”. However, v2.1.4 has been public for about a year. While changing the version of the pipeline is probably not required, I recommend removing the word “latest”
    
    Response : Fixed. 
    
    2. Lines 142-149: It is unclear why the paper chose to use both tbabs and tbnew. This needs to be expanded upon and better justified.
    
    Response : Tbabs is a primitive model with reasonable assumptions and could be used with Galactic absorption. Tbnew includes the column density of other elements, as it could be useful for sources with high absorption. We used Tbnew in all the cases except for V404 where the variability is quantified by the flux-resolved spectroscopy and removing the highly absorbed flux in the energy range of 7.5-8.0 keV where the absorption is observed. It has been mentioned in the text at the beginning of Section 3. 


    3. Line 242: I suspect that was a typo, especially seeing how the paragraph after discusses the emissivity profile. This sould probably have been relxillCp_nk and not relxilllpCp_nk
    
    Response: Fixed.
    
    4. Lines 244-247: Complex residuals above 40 keV cannot be attributed to absorption. Absorption effects would be dominant at low energies.
    
    REsponse" Corrected.
    
    5. Lines 259-260: “the reflection fraction value of less than 1 implies that the spectra is dominated.” This sentence likely misses the messages that the authors meant to include
    
    Response: Fixed.
    
    6. Line 301: Fixing the Fe abundance to 10 strongly tightens the uncertainties on all the other parameters. Also, a value of 10 is unphysical. 
    
    Response: The iron abundance is constrained and pegged at 10 during the fit. This freezing of iron abundance is supported in the literature (Mori et al. 2019), where Fe is also fixed at 10. It does not affect the fit if the iron abundance is fixed at any value. The errors are very small, as they are statistical.
    
    7. Line 302-304: It is not clear how/why a reflection fraction of 0.37 implies that the spectra are reflection-dominated. What does it mean to be reflection-dominated? Would we not expect that for a reflection fraction greater than 1?
    
    Response: We have fixed the statement and added some text in line 325. 
    
    8. Line 308: the uncertainty of +0.0005 is likely meaningless. Please see the points above. With half of the parameters frozen, the uncertainty will be artificially reduced.
    
    Response : In this case, the higher bound is not calculated properly as the highest value of spin is fixed at 0.998. In MCMC simulations, many values are accumulated nearer the higher bound and affected the distribution of the parameter. Now, we show only the lower bound of the measurement. 
    
    9. Lines 368-370: if the column density of the xstar model is higher for the second half of the observation and all the other parameters are consistent, why does the flux go up during the second half? A higher column density would cause a lower flux.
    
    Response : The emissivity profile of part I observation is well fitted by broken power law whereas for part II, single power law describes the emissivity. Therefore broken power law, with inner emissivity index of 10, would accumulate more emission in the inner region of the black hole, causing the reflection from the disk to increase. After the break radius of 7 , the emissivity index becomes 3 which is the Newtonian profile. However, for part II, the single power law with inner emissivity of ~10, similar to $q_{in}$ of part I, is same throughout the disk which results in the increase of ionization of the relativistic reflection and warm absorber around it. We have added this explanation in the text (lines 396-405). 
    
    10. Lines 392-398: This paragraph needs many references.
    
    Response: Added. 
    
    11. Lines 399-401: Why is the analysis focused on only one observation? Would it not make more sense to analyze all observations of a single source and see how the spin & alpha vary across observations? Especially seeing how the spin should be constant. 
    
    Response: We selected observations where the iron line is clearly visible. It is not necessary that the iron line is prominent for all the observations of the source. We only select the observation which has been well studied in the past so that we can test the Kerr metric for the analyzed observation. 
    
    12.	Line 407: “don’t” -> do not 
    
    Response: Fixed. 
    
	13.	Line 445: please check the value listed of 110ks. The light curve in Figure 7a shows 100ks, and given that the exposure was not continuous, I suspect that the 110ks number should be much smaller.
    
    Response: For the flux state 1, the exposure time is 1.4 ks which is now included in the text. 
    
	14.	Throughout the paper, a lot of sentences start with “So, ...” This is very informal and should probably be avoided. 
    
    Response: Fixed.
    
	15.	Lines 483-486: Using xillver (emission) to account for an edge (absorption) is plain  wrong. Edges are caused by absorption, and one should either use the appropriate model to explain the “edge”. However, I suspect that the authors did not actually identify an “edge” - the closest important one would be the Fe K alpha edge at 7.1 keV. I suspect that the spectra simply showed residuals that resembled that. The text should clarify this aspect.  It is not only the edge but other absorption which fit nicely with xillver supported by the more increase in chi-square than edge alone. 
    
    Response: We are thankful to referee for this comment. We fixed the statement in the manuscript (lines 573-576). 
    
	13.	Lines 632-633: “we select the best profile yielding minimum chi2 likelihood.” The text should either say minimum chi2 or maximum likelihood, but not combine the two. Also, this sentence should be stated much earlier in the paper, likely in Section 2 or at the beginning of Section 3.  
    
    Response: We have fixed this in the manuscript (line 652) and also state it earlier in section 3 on page 4, just before the results of T15 (line 221). 
    
	14.	Line 602: the paper mentions the B1 model, but that is not mentioned anywhere else in the paper. Please clarify. 
    
    Response: We have changed the B1 model to the best-fit model. 
    
	15.	Line 643: the model nbkk is never mentioned in the paper previously and should be explained. 
    
    Response: We now remove the nkbb model from the text as it is not necessary and haven't been mentioned anywhere else in the manuscript. 
    
	16.	Lines 649-652: This argument is not convincing. The claim that emission from within the plunging region does not matter for these sources because of their high spins and therefore low ISCOs is circular. The idea is that if the emission from within the plunging regions did, in fact, matter, sources with low spins would have significant emission from within the ISCO and produce spectra that would look like having been caused by high spins, meaning that past results claiming that these BHs are rapidly rotating are wrong. If radiation from within the ISCO matters, we cannot trust past measurements of high spins. 
    
    Response: We are thankful to referee for the suggestion and fixed this statement in the discussion section (lines 726-732).
    
	17.	Lines 668-671: This paragraph has no use in its current shape. The paper would benefit from a stronger conclusion, discussion of tangible future projects, the implications of the work, how instruments such as Athena would help the field, what needs to happen with the models, etc. Currently, it serves as a filler to end the text. 
    
    Response: We have now included conclusions from the paper in this paragraph.
    
    18.	Figure 9: The legend and y label are confusing. I would suggest replacing the y label to “ratio” and having the legend simply read alpha=-0.4 etc. instead of alpha=-0.4/alpha=0 - the two consecutive equal signs are confusing. 
    
    Response: The modified figure is added in the manuscript.
    
	19.	Figure 10: the error bars for the points in this version of the figure shrunk significantly compared to the previous version. Why? Previously, the figure has some shift in the sources’ name. 
    
    Response: There was some plotting error in the earlier version which is now fixed. We also updated the constraints of the sources analyzed in this work. Now, the constraints are similar to those plotted in Tripathi et al. 2021b. 
    
	20.	Figure 11: this figure would benefit from including the residuals to the fit. Also, the figure should not plot “eeufspec” but rather “ldata” or “eedata” (this new command was added in recent versions of xspec). 
    
    Response: The effect of the warm absorber on the fit is too small to be seen in any residual or eedata plot. We plot eeufspec because it makes the features, as the referee mentioned, "impressive". So, we used eeufspec to show the effect of a warm absorber. The warm absorber is added for two reasons: improvement in chi-square and attainment of constrained parameters. So, we requested the referee to let us keep these eeufspec plots in the paper. 
    
	21.	Table 3: With both T15 and T37 being close to the galactic center, why is the column density in tbabs so different between the two? 
    
    Response: It is not necessary for the column density to be the same for nearby sources. It also depends on the absorption along the line of sight, which could potentially be different for two nearby sources. Besides, these values are consistent with those found in the literature. 
    
	22.	Table 3: Why does the reflection fraction for the two halves of the MAXI J1631 observation change from 6 to 1?
    
    Response: It could be due to different emissivity profiles found for different parts of the observations which also affect the ionization of relxill\_nk and warm absorber. We have added text about this on page 8 (lines 396-405). 
    
	23.	Table 4: why does kT_e drop from 400 keV to 40 keV between spectra? 
    
    Response: They are different sources. So, it is possible that kT_e is different. 
    
	24.	Tables 3&4: the normalizations of the components should be included in the tables.
    
    Response: Normalizations of the components are added to the tables.  
    
	25.	Line 669: Please replace the reference for Athena with NewAthena (Cruise et al. 2025)
    
    Response: Done
    
	26.	Line 646: please provide references for the statement that the assumption of the disk extending to the ISCO is valid for that Eddington ratio range. 
    
	Response: Added. 
    
	27.	Please discuss the interesting behavior in the alpha_13 - spin panel in the left corner plot of Figure 6. What is causing this bimodal distribution? What does chi2 look like in comparison to those? I.e. spin vs chi2, alpha_13 vs chi2? 
    
    Response: The bimodal distribution shows that they are likely two solutions for alpha13 or we need more simulations to clarify whether this bimodality is the consequence of some statistical limitation which is beyond the scope of the work. We have added this explanation in the text (lines 427-436). 
    
	28.	Caption of figure 3: multiple instances of double parentheses 
    Response: Fixed. 
    
	29.	The abstract should expand on the work, present the results, and mention the  importance of the findings. 
	Response : The abstract is modified.


New report 

 Referee report on “Testing General Relativity with NuSTAR data of Galactic Black Holes: II”
Before responding, I want to assure the authors that my intention as a reviewer is to help improve the paper, both in terms of quality and future impact. While I sympathize with the desire to have a paper published in a timely manner, I consider that there are still several aspects of the paper that should be addressed.
First and foremost, this point comes more from the perspective of a scientist than that of a reviewer. I consider that the paper would strongly benefit from a better contextualization of the intended science objective. I understand that in past work, the authors performed this sort of work on 6 systems, and in this work, they add 4 more. I understand that these 4 sources are heavily obscured (complicated spectra). However, the newly added paragraph just before Section 2.1 does not justify the impact of the paper.
The claim is that this paper demonstrates that such a measurement can be performed in “complicated” systems. However, all these spectra have been analyzed before, and all the original works find good fits. The paper does not demonstrate its need/novelty, as it takes already analyzed data, and performs an analysis with a model with an extra free parameter, to demonstrate that this extra free parameter is not needed. We knew that this was not needed from the original analysis. Currently, all the paper does is to recover old results. I understand that the idea is to expand the analysis to obscured sources, but saying that this was done to show that it is possible does not represent a convincing justification for such an analysis.
To be clear: I am not criticizing the idea of probing deviations from the Kerr metric. I think this is valuable, and the fact that all the fits produce values of alpha_13 consistent with 0 is still important information. However, I consider that the paper would benefit from a rework of the story that it is trying to present. I consider that this would also increase the visibility and the future impact of the paper. A few examples of points that the authors could consider for better contextualizing the paper include: 1) What values of alpha_13 does the data definitively exclude? 2) What do we need to understand the systematic uncertainties, and how do those compare with the statistical uncertainties? 3) How many measurements do we need to place definitive constraints for/against the Kerr metric? 4) What exactly would data from Athena do to enhance the field? 5) Why is it important/relevant to perform such analysis on “complicated” sources? Why do we care about doing this in heavily obscured sources? Demonstrating answers to all/some of these questions would help contextualize the paper, make it relevant to more people, increase its visibility, and ultimately its impact.
Response : We are really thankful to the referee for such suggestions which improves the quality of the manuscript. We have added the following information at the end of the discussion section. 

"The analysis using relxill\_nk is more than merely fitting the data with relxill, having one extra parameter. It is physically motivated in the sense that the value of this extra parameter, which is $\alpha_{13}$, signifies the presence of a non-Kerr spacetime near the inner-most region of the black hole. At the very least, allowing for such a deformation can absorb potential systematic uncertainties in the astrophysical and spectral models. By introducing an additional degree of freedom beyond the standard models, we gain the ability to probe such systematics explicitly. The statistical uncertainty on the deformation provides a quantitative measure of how much the true spacetime or modeling uncertainties might deviate from theoretical predictions. The statistical uncertainty should become smaller with the future instruments like NewAthena \citep{2025NatAs...9...36C} with high resolution spectroscopy while any systematic biases in models might remain. Such analyses therefore allow us not only to constrain possible deviations, but also to quantify systematic biases in reflection models.

In \citet{2021ApJ...913...79T}, simple sources are analyzed where the absorption is negligible, and therefore, the systematics are limited. The observations analyzed in this work have systematics due to heavy absorption, in addition to the usual systematics associated with the reflection model discussed previously. In this work, we reduce the systematics due to heavy absorption by sophisticated data reduction and analysis techniques and successfully constrain $\alpha_{13}$ between -1.0 and 0.5 which includes the Kerr solution. Getting consistent zero deformation values signify that even with the complicated spectra, the models work well for the data quality of \textsl{NuSTAR}. \citet{Tripathi:2020dni} addresses the systematics due to the reflection model by analyzing data with different models which is beyond the scope of this work. 

Measuring deviations from the Kerr metric is one way to falsify the underlying theory. To date, all observational results are consistent with Kerr within statistical errors. If we ever observe a statistically significant deviation, it may not simply mean GR is incorrect. Rather, it would open the possibility of exploring more intricate physics through improved theoretical models and observational techniques. Even then, demonstrating a deviation from Kerr would help us challenge or refine our understanding of the spacetime metric. The more such observations are found in X-ray and in other techniques, the stronger our conclusions about the spacetime geometry will become.

This paper attempts to address the systematics due to the reflection model and heavy absorption, and still demonstrate the capability of X-ray reflection spectroscopy to constrain the deviations from the Kerr metric. These four measurements open a new frontier, showing that absorbed sources can also be employed to test the Kerr hypothesis.  Although these results do not provide the existence of a non-Kerr black hole, it assuredly strengthens the claim of these objects being described by the Kerr metric, which is also a confirmation of the assumption of explaining the space-time metric with the Kerr metric in most of the relativistic reflection models currently employed in X-ray astronomy. The future X-ray telescopes, like \textsl{eXTP} \citep{Zhang:2016ach} and \textsl{NewAthena} \citep{2025NatAs...9...36C}, would provide a higher energy resolution around the iron line. This improved sensitivity will prove helpful in obtaining stringent constraints on non-Kerr metric."

I hope this text would provide a convincing justification to the analysis done in this work and also improves its visibility and impact. 
 
We also added some information about the other tests of gravity using Gravitational waves and Event Horizon Telescope on page 2 (lines 84-89)

In addition to this broad suggestion, there are a number of small issues that must be addressed, which are outlined below. Please note that all these suggestions refer to newly added text or to points from the previous report that were not properly addressed.
1. Figure 11: I would recommend replacing the y label to read “ratio.” In its current form, the plot does not make it clear that it shows a ratio of spectral models, and one needs to look in the figure caption to find that.
Response: We have modified the figure in the manuscript. 

 2. Figure 12: MAXI J1631-479 has two dashes in its name - please correct. Additionally, I consider that it would benefit this figure to write out the full names of T15, T37, and V404. The reason for that is to make the figure more applicable to use by others in talks etc., without the need to explain what those labels are. It makes it easier for the community to use this plot in the future, and increases the visibility of this paper.
Response: We have included the full names of the sources in the modified plot. 
 
3. Line 727: matter -> matters
Response: Fixed at line 749. We have also added text about the recent results about the plunging region in lines 752-755. 

4. Line 748: till -> until
Response: Fixed.

5. Line 748: explain what “simple” sources are
Response: Explained in the text on line 787. 

6. Line 754: “observations observed” sounds awkward. Please rephrase
Response: We have rephrased the whole paragraph. 

7. Line 755: “If not the non-Kerr, it ...” This sentence is unclear. Please rephrase
Response: We have rephrased the statement and the whole paragraph. 

8. Line 644: It seems like a sentence is missing here before “each time.” It would make
sense to say something about how after the initial fit with alpha_13=0, the value is
allowed to vary freely, and then that the chi2 improves
Response:  We fixed the sentence (line 663). 

9. Table 4: as asked in the previous version of the report, why do the values of kTe change
from 400 to 40? The authors responded that these are different sources. That is not true
- all these spectra are of V404. The different sources are in Table 3.
Response: We are thankful to the referee for pointing out this anomaly. In the chi-square best fit result in xspec, these two values of kTe are unconstrained and only have upper bound. In MCMC, these parameters are constrained on the value of their upper bound. We have now corrected the measurement and show only the upper bound in the table. 

10. Line 390: Figure 6 does not definitively demonstrate the need for the warm absorber. In
its current state, figure 6 shows what the model looks like with and without the warm absorber. However, even without it, the model goes through all the data points. From that perspective, this figure does not demonstrate the need for the warm absorber - it only shows what the model looks like with or without. I strongly believe that a figure akin to 2 or 3 would help demonstrate the need for the warm absorber. I understand wanting to plot eeufspec, but try to plot eedata too (even if it’s not included in the paper) and the residuals too.
Response: We have now attached the eedata and residuals for the part 1 observation of MAXI J1631, as in figure 6 (part1_eemodel.ps with warm absorber and part1_eemodel+nowa.ps without warm absorber). In residuals, there are minor differences around 5-7 keV, which is very difficult to visualize in the eedata plot. We would respectfully like to keep the eeufspec plot in the manuscript as it will show the difference in a more pronounced manner. 

11. Line 349-351: the newly added text needs references supporting these statements. Personally, I can think of significantly more literature pointing to the disk extending to the ISCO in the hard state than to truncation, but that is beyond the scope of this paper. Nevertheless, whichever stance the authors take, it needs to be properly backed by existing literature.
Response: We have added two references to support these statements. Besides, we also added a footnote about the simulations related to plunging region. 

12. Lines 162-165: the newly added text is confusing. It is unclear what is being removed and how that relates to tbnew.
Response: We are thankful to the referee for addressing this issue. Indeed the sentence is confusing and is now corrected (line 178). We have omitted the statement after "and". 

13. Line 135: “we demonstrate” -> “we aim to demonstrate”
Response: Fixed in the manuscript (line 151). 

14. Line 128: remove “s” at the end of “meets” and add “the” after “testing”
Response: Done (line 132). 

15. Lines 130-134: the sentence starting with “in Marinucci et al 2014” seems out of place.
That paper is not explained, and in the current form, this reference seems like a filler.
Please revise, especially in the context of the initial comment.
Response: We have explained the paper briefly and revised the statement (lines 136-149). 

16. In the previous report, it was pointed out that a lot of sentences start with “So, ...” and that this should be changed. The authors said that this was fixed. There are still 6
instances of sentences starting that way. Please address.
Response: We have fixed all such instances in the manuscript. 

17. Regarding the prior point 6, related to the Fe abundance being fixed at 10. The authors
say that this value is backed by archival work (Mori et al 2019). While this argument is not strong, it is acceptable. However, saying that the fit is unaffected if the Fe abundance is fixed to any value is likely false. Even so, if true, why fix it to 10 and not 1?
Response: When Fe is free to vary, its value gets pegged at 10. So, we decided to freeze it at 10 and continue with the analysis. We have mentioned this in the text (line 339). 
